Impact of Short Blocklength Coding on Stability of an AGV Control System in Industry 4.0

With the advent of 5G and beyond, using wireless communication for closed-loop control and automation processes is one of the main aspects of the envisioned Industry 4.0. In this regard, a major challenge is to ensure a robust and stable control system over an unreliable wireless channel. One of the main use-cases in this context is Automated Guided Vehicle (AGV) control in a future factory. Specifically, we consider a system where an AGV controller is placed in an edge cloud in the factory network infrastructure and the control commands are sent over a time-correlated Rayleigh fading channel. In an industrial control, short packets are exchanged between the controller and the actuator. Therefore, in this case, Shannon's assumption for an infinite block length is not applicable. The objective is to analyse the stability performance of an AGV control system in a Finite Block-Length (FBL) regime. We evaluate the coding rate required to maintain a stable edge cloud based AGV system. The results illustrate that adapting the control parameters can lower the stringent requirements on the coding rate. It reveals that a constant stability performance can be achieved even at higher coding rate by increasing the AGV's velocity. Moreover, this paper also determines the maximum number of AGVs that can be served seamlessly over the available communication resources while maintaining a stable control system.

==> Results/Pb_R.tex <==
\begingroup
\unitlength=1mm
\psset{xunit=65.00000mm, yunit=62.50000mm, linewidth=0.1mm}
\psset{arrowsize=2pt 3, arrowlength=1.4, arrowinset=.4}\psset{axesstyle=frame}
\begin{pspicture}(-0.23077, -0.25600)(1.00000, 0.80000)
\rput(-0.03077, -0.08000){%
\psaxes[subticks=0, labels=all, xsubticks=1, ysubticks=1, Ox=0, Oy=0, Dx=0.2, Dy=0.2]{-}(0.00000, 0.00000)(0.00000, 0.00000)(1.00000, 0.80000)%
\multips(0.20000, 0.00000)(0.20000, 0.0){4}{\psline[linecolor=black, linestyle=dotted, linewidth=0.2mm](0, 0)(0, 0.80000)}
\multips(0.00000, 0.20000)(0, 0.20000){3}{\psline[linecolor=black, linestyle=dotted, linewidth=0.2mm](0, 0)(1.00000, 0)}
\rput[b](0.50000, -0.17600){$\text{Coding Rate} \: \left(R \right) \: \left[ \unit{bits per c.u} \right] $}
\rput[t]{90}(-0.20000, 0.40000){$\text{Avg. Prob. of block error} \left( EPblk\right) $}
\psclip{\psframe(0.00000, 0.00000)(1.00000, 0.80000)}
\psline[linecolor=blue, plotstyle=curve, linewidth=0.4mm, showpoints=false, linestyle=solid, linecolor=blue, dotstyle=o, dotscale=1.2 1.2, linewidth=0.4mm](1.00000, 0.89794)(0.50000, 0.73348)(0.33333, 0.62548)(0.25000, 0.54976)(0.20000, 0.49317)(0.16667, 0.44894)(0.14286, 0.41322)(0.12500, 0.38364)(0.11111, 0.35866)(0.10000, 0.33724)(0.09091, 0.31862)(0.08333, 0.30225)(0.07692, 0.28774)(0.07143, 0.27476)(0.06667, 0.26308)(0.06250, 0.25249)(0.05882, 0.24285)(0.05556, 0.23402)(0.05263, 0.22591)(0.05000, 0.21842)(0.04762, 0.21148)(0.04545, 0.20504)(0.04348, 0.19903)(0.04167, 0.19342)(0.04000, 0.18816)(0.03846, 0.18322)(0.03704, 0.17857)(0.03571, 0.17419)
\psline[linecolor=red, plotstyle=curve, linewidth=0.4mm, showpoints=true, linestyle=solid, linecolor=red, dotstyle=diamond, dotscale=1.2 1.2, linewidth=0.4mm](1.00000, 0.89587)(0.50000, 0.72814)(0.33333, 0.61971)(0.25000, 0.54510)(0.20000, 0.49006)(0.16667, 0.44738)(0.14286, 0.41310)(0.12500, 0.38482)(0.11111, 0.36100)(0.10000, 0.34059)(0.09091, 0.32287)(0.08333, 0.30731)(0.07692, 0.29350)(0.07143, 0.28115)(0.06667, 0.27002)(0.06250, 0.25993)(0.05882, 0.25072)(0.05556, 0.24228)(0.05263, 0.23451)(0.05000, 0.22733)(0.04762, 0.22066)(0.04545, 0.21446)(0.04348, 0.20866)(0.04167, 0.20324)(0.04000, 0.19814)(0.03846, 0.19335)(0.03704, 0.18883)(0.03571, 0.18456)
\endpsclip
\psframe[linecolor=black, fillstyle=solid, fillcolor=white, shadowcolor=lightgray, shadowsize=1mm, shadow=true](0.53846, 0.64800)(0.92308, 0.80000)
\rput[l](0.67692, 0.75200){\footnotesize{$\text{v=1m/s}$}}
\psline[linecolor=blue, linestyle=solid, linewidth=0.3mm](0.56923, 0.75200)(0.63077, 0.75200)
\rput[l](0.67692, 0.69600){\footnotesize{$\text{v = 20m/s}$}}
\psline[linecolor=red, linestyle=solid, linewidth=0.3mm](0.56923, 0.69600)(0.63077, 0.69600)
\psline[linecolor=red, linestyle=solid, linewidth=0.3mm](0.56923, 0.69600)(0.63077, 0.69600)
\psdots[linecolor=red, linestyle=solid, linewidth=0.3mm, dotstyle=diamond, dotscale=1.2 1.2, linecolor=red](0.60000, 0.69600)
}\end{pspicture}
\endgroup
\endinput

